GS-Blur: A 3D Scene-Based Dataset for Realistic Image Deblurring

To train a deblurring network, an appropriate dataset with paired blurry and sharp images is essential. Existing datasets collect blurry images either synthetically by aggregating consecutive sharp frames or using sophisticated camera systems to capture real blur. However, these methods offer limited diversity in blur types (blur trajectories) or require extensive human effort to reconstruct large-scale datasets, failing to fully reflect real-world blur scenarios. To address this, we propose GS-Blur, a dataset of synthesized realistic blurry images created using a novel approach. To this end, we first reconstruct 3D scenes from multi-view images using 3D Gaussian Splatting (3DGS), then render blurry images by moving the camera view along the randomly generated motion trajectories. By adopting various camera trajectories in reconstructing our GS-Blur, our dataset contains realistic and diverse types of blur, offering a large-scale dataset that generalizes well to real-world blur. Using GS-Blur with various deblurring methods, we demonstrate its ability to generalize effectively compared to previous synthetic or real blur datasets, showing significant improvements in deblurring performance.

==> sections/figures/realiability.tex <==
\begin{figure}[t]
    \renewcommand{\wp}{0.125\linewidth}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{minipage}[c]{0.1 \linewidth}
    \vspace{-1.0cm}
    \makecell{\scriptsize GT~\cite{yu2023mvimgnet}}
    \\
    \end{minipage}
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \\
    \vspace{-8mm}
    \begin{minipage}[c]{0.1 \linewidth}
    \vspace{-1.2cm}
    \makecell{\scriptsize Rendered\\ \scriptsize (\textbf{GS-Blur})}
    \\
    \end{minipage}
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{figures/figure1/6_02_0e0128f5_15_r2_0.7_0.png}}
    \vspace{-4mm}
    \caption{\textbf{Visualization of the ground truth from MVImgNet~\cite{yu2023mvimgnet}~(top) and our rendered sharp images~(bottom).}
    The sharp images, closely matching the ground truth images from MVIMGNet, serve as the target sharp images in the GS-Blur dataset.
    }
    \label{fig:reliability}
    \vspace{-1mm}
\end{figure}


==> sections/figures/rigid.tex <==
\begin{figure}[t]
    \renewcommand{\wp}{0.12\linewidth}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{minipage}[c]{0.08 \linewidth}
    \makecell{$\mathbf{T}_{obj}$}
    \\
    \vspace{0.5cm}
    \end{minipage}
    \hspace{8mm}
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \\
    \vspace{-8mm}
    \begin{minipage}[c]{0.08 \linewidth}
    \makecell{$\mathbf{T}_{bg}$}
    \\
    \vspace{0.5cm}
    \end{minipage}
    \hspace{8mm}
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \\
    \vspace{-8mm}
    \begin{minipage}[c]{0.08 \linewidth}
    \makecell{$\mathcal{B}(\mathbf{T}_{obj}, \mathbf{T}_{bg})$}
    \\
    \vspace{0.5cm}
    \end{minipage}
    \hspace{8mm}
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \hfill
    \subfloat[]{\includegraphics[width=\wp]{example-image-duck}}
    \vspace{-8mm}
    \caption{Visualization of randomly generated 3D trajectories~$\mathbf{T}_{obj}$ for the object and $\mathbf{T}_{bg}$ for the background, along with their corresponding motion-blurred images~$\mathcal{B}(\mathbf{T}_{obj, \mathbf{T}_{bg}})$.
    }
    \label{fig:rigid}
\end{figure}



==> sections/tables/add_dataset.tex <==
\begin{figure}[t]
\captionsetup[subfigure]{labelformat=empty}
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/1/000133.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/1/GOPR0410_11_00_000133.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/1/ours1.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/1/000133_gt.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/2/005_00000095.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/2/reds.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/2/ours2.png}}
  \hfill
  \subfloat[]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/2/005_00000095_gt.png}}
  \vspace{-8mm}
  \\
\captionsetup[subfigure]{labelformat=parens}
\addtocounter{subfigure}{-8}    
  \subfloat[\tiny Input]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/3/BSD_3ms24ms_091_00000093_blur.png}}
  \hfill
  \subfloat[\scriptsize Prev.]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/3/bsd.png}}
  \hfill
  \subfloat[\scriptsize +\textbf{GS-Blur}]{\includegraphics[width=0.12\linewidth]{figures/add_ours/3/ours3.png}}
  \hfill
  \subfloat[\scriptsize GT]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/3/BSD_3ms24ms_091_00000093_gt.png}}
  \hfill
  \subfloat[\scriptsize Input]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/4/avg_blur.png}}
  \hfill
  \subfloat[\scriptsize Prev.]{\includegraphics[width=0.12\linewidth]{figures/add_ours/4/rsblur.png}}
  \hfill
  \subfloat[\scriptsize +\textbf{GS-Blur}]{\includegraphics[width=0.12\linewidth]{figures/add_ours/4/ours4.png}}
  \hfill
  \subfloat[\tiny GT]{\includegraphics[width=0.12\linewidth]{figures/add_ours2/4/0002_001504_gt.png}}\\
\caption{
\textbf{Visual comparison between model trained on multiple sources with and without GS-Blur.}
Prev. refers to GoPro+REDS+BSD+RSBlur, and +GS-Blur denotes networks trained with both prev. and our proposed GS-Blur.
The samples are sourced from GoPro, REDS, BSD, and RSBlur, respectively.
% For (c), (g), (k), and (o), we train the model using (b), (f), (j), (n), and GS-Blur, respectively. \joon{revise all!}}
}
\label{fig:add_dataset}
\vspace{-2mm}
\end{figure}


==> sections/tables/all.tex <==
\begin{table}[!t]
% \centering
% \begin{minipage}{0.43\linewidth}
% % \setlength\tabcolsep{0pt}
% \captionof{table}{
% \textbf{Quantitative comparison by using GS-Blur alongside existing datasets.}
% % We evaluate metrics consistent with the trained sets.
% }
% \label{tab:add_dataset}
% \centering
%    \resizebox{0.53\linewidth}{!}{
%    \begin{tabular}{c|cc}
%     \toprule
%     Train Set & PSNR & SSIM \\
%     \midrule
%     GoPro & 32.81 & \textbf{0.960} \\
%     GoPro + \textbf{GS-Blur} & \textbf{33.89} & \textbf{0.960} \\
%     \midrule
%     REDS & 33.49 & 0.946\\
%     REDS + \textbf{GS-Blur} & \textbf{33.79} & \textbf{0.949}\\
%     \midrule
%     BSD & 33.87 & \textbf{0.953}\\
%     BSD + \textbf{GS-Blur} & \textbf{33.88} & \textbf{0.953} \\
%     \midrule
%     RSBlur & 33.83 & 0.907\\
%     RSBlur + \textbf{GS-Blur} & \textbf{34.11} & \textbf{0.909} \\
%    \bottomrule
%   \end{tabular}}
% \end{minipage}
% \hfill
\centering
\caption{
\textbf{Quantitative comparison between model trained on multiple sources with and without GS-Blur.}
As shown, deblurring performance consistently improves across various benchmark datasets when the model is additionally trained on our GS-Blur.
}
\label{tab:all_validation}
\smallskip
\resizebox{0.82\linewidth}{!}{
\begin{tabular}{lc|cccc}
\toprule
Train Set & Test set & GoPro & REDS & BSD & RSBlur \\
\midrule
\multirow{2}{*}{GoPro + REDS + BSD + RSBlur} & PSNR & 32.67 & 32.49 & 33.47 & 33.50\\
& SSIM & 0.958 & 0.935 & 0.949 & 0.886\\
\midrule
\multirow{2}{*}{GoPro + REDS + BSD + RSBlur + \textbf{GS-Blur}} & PSNR & \textbf{32.79} & \textbf{32.83} & \textbf{33.62} & \textbf{33.76} \\
& SSIM & \textbf{0.960} & \textbf{0.940} & \textbf{0.951} & \textbf{0.890}\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\end{table}


==> sections/tables/overall.tex <==
\begin{table}[t]
\newcommand{\cmark}{\textcolor{MyGreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{MyRed}{\ding{55}}}%
\newcommand{\trimark}{\textcolor{blue}{\ding{115}}}
\centering
  \caption{
  \textbf{AAA}
  }
  \label{tab:overview}
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l|c|c|c|c}
    \toprule
    Dataset & Realistic blur? & Diverse blur trajectories? & Diverse camera models? & Large scale?\\
    \midrule
    GoPro & \xmark & \trimark & \xmark & \xmark \\
    REDS & \xmark & \trimark & \xmark & \xmark \\
    BSD & \cmark & \trimark & \xmark & \xmark \\
    RSBlur & \trimark & \trimark & \trimark & \xmark\\
    GS-Blur~(Ours) & \xmark & \cmark & \cmark & \cmark\\
   \bottomrule
  \end{tabular}}
\end{table}

